Exact solutions of open integrable quantum spin chains

In the thesis we present an analytic approach towards exact description for steady state density operators of nonequilibrium quantum dynamics in the framework of open systems. We employ the so-called quantum Markovian semi-group evolution, i.e. a general form of time-autonomous positivity and trace-preserving dynamical equation for reduced density operators, by only allowing unitarity-breaking dissipative terms acting at the boundaries of a system. Such setup enables to simulate macroscopic reservoirs for different values of effective thermodynamic potentials, causing incoherent transitions between quantum states which are modeled with aid of the Lindblad operators. This serves as a simple minimalistic model for studying quantum transport properties, either in the linear response domain or in more general regimes far from canonical equilibrium. We are mainly exploring possibilities of identifying nonequilibrium situations which are amenable to exact description within matrix product state representation, by exclusively focusing on steady states, i.e. fixed points of the Lindblad equation, of certain prototypic interacting integrable spin chains driven by incoherent polarizing processes. Finally, we define a concept of pseudo-local extensive almost-conserved quantities by allowing a violation of time-invariance up to boundary-localized terms. We elucidate the role of such quantities on non-ergodic behaviour of temporal correlation functions rendering anomalous transport properties. It turns out that such conservation laws can be generated by means of boundary universal quantum transfer operators of the fundamental integrable models.

==> App_Hopf.tex <==
\chapter{Hopf algebras and quantum groups.}
\label{sec:App_Hopf}

In this section we use notation which stands on its own right.
Let $\cal{A}$ be a unital associative algebra over $\CC$ with linear maps
\begin{itemize}
 \item $m:\cal{A}\otimes \cal{A}\rightarrow \cal{A}$ (multiplication)
 \item $\eta:\CC \rightarrow \cal{A}$ (unit).
\end{itemize}
Multiplication map,  $m(x\otimes y)=xy$, is \textit{associative}, $m((m(x\otimes y))\otimes z)=m(x\otimes m(y\otimes z))$ for all $x,y,z\in \cal{A}$. Existence of
unit implies $\eta(1)=\one$, $\one \in \cal{A}$.
Those objects admit a very natural dual construction, which gives rise to \textit{coalgebra} $\cal{C}$ (over $\CC$), i.e. we have linear maps
\begin{itemize}
 \item $\Delta:\cal{C} \rightarrow \cal{C}\otimes \cal{C}$ (comultiplication or coproduct)
 \item $\epsilon:\cal{C}\rightarrow \CC$ (counit).
\end{itemize}
A coproduct is \textit{coassociative},
\begin{equation}
(\Delta \otimes \id)\circ \Delta=(\id \otimes \Delta)\circ \Delta.
\label{eqn:coassociativity}
\end{equation}
Both sides are maps from $\cal{C}\rightarrow \cal{A}\otimes \cal{C}\otimes \cal{C}$. This property allows for extension to multiple product spaces.
Using Sweedler's notation in expansion of a coproduct, $\Delta(x)=\sum_{i}x^{i}_{1}\otimes x^{i}_{2}\equiv x_{1}\otimes x_{2}$, the
coassociativity compactly reads $\Delta(x_{1})\otimes x_{2}=x_{1}\otimes \Delta(x_{2})$, for all $x\in \cal{A}$. Counit fulfills
\textit{counitarity} condition, $\epsilon(\one)=1$.
Combination of algebra $(\cal{A},m,\eta)$ with a coalgebra $(\cal{C},\Delta,\epsilon)$ defines a
\textit{bialgebra} $\cal{H}$ $(\cal{H},m,\eta,\Delta,\epsilon)$, provided the stuctures $m,\eta$ of  are compatible with $\Delta,\epsilon$.

If in addition a bialgebra $\cal{H}$ is endowed by an antimultiplicative linear map
\begin{itemize}
 \item $S:\cal{H}\rightarrow \cal{H}$ (antipode or coinverse),
\end{itemize}
we obtain a \textit{Hopf algebra}. Beside coassociativity, the co-strucutures obey
\begin{align}
(\id \otimes \epsilon)\Delta(x)&=(\epsilon \otimes \id)\Delta(x)=x,\\
m(S\otimes \id)\Delta(x)&=m(\id \otimes S)\Delta(x)=\epsilon(x)\one,
\label{eqn:costructures}
\end{align}
and multiplicative properties
\begin{align}
\Delta(xy)&=\Delta(x)\Delta(y),\quad \Delta(\one)=\one \otimes \one \\
\epsilon(xy)&=\epsilon(x)\epsilon(y),\quad \epsilon(\one)=1\\
S(xy)=S(y)S(x),\quad S(\one)=\one.
\label{eqn:multiplicative}
\end{align}
It is noteworthy that the antipode acts like an inverse, although it is not restricted to $S^{2}=\id$.

Definition of a Hopf algebra can be nicely expressed in terms of a commutative diagram.
% draw a diagram as e.g. http://en.wikipedia.org/wiki/Hopf_algebra

\paragraph{Universal enveloping algebra $\cal{U}(\frak{g})$.}
Below we provide a simple example of a Hopf algebra. Imagine a Lie algebra $\frak{g}$, given in terms of the generators $\xi_{i}$,
\begin{equation}
[\xi_{i},\xi_{j}]=C^{ij}_{k}\xi_{k}.
\label{eqn:Lie_algebra_structure}
\end{equation}
This is \textit{not} a unital associative algebra. However algebra $\frak{g}$ admits a natural extension to an algebra $\cal{U}(\frak{g})$,
called a \textit{universal enveloping algebra}, which is characterized by $\frak{g}$. First, construct a \textit{tensor algebra} (or a \textit{free algebra}),
\begin{equation}
\cal{T}(\frak{g})=\bigoplus_{n\geq 0}\frak{g}^{\otimes n},
\label{eqn:tensor_algebra}
\end{equation}
which is just an algebra with unit and words of generators $\xi_i$ from $g$ of all lengths. Then, take a two-sided ideal generated by $\frak{g}$
\begin{equation}
\cal{I}=x\otimes y-y\otimes x-[x,y],
\label{eqn:ideal}
\end{equation}
and define $\cal{U}(\frak{g}):=\cal{T}(\frak{g})/\cal{I}$. In words, UEA is a free algebra of strings of generators from $\frak{g}$ modulo Lie-algebra
commutation relations. By Poincar\'{e}-Birkhoff-Witt theorem (PWB) a basis of $\cal{U}(\frak{g})$ consists of all ordered monomials in the
generators $\xi_i$. Moreover, $\cal{U}(\frak{g})$ can be assigned a simple Hopf algebra structure, by introducing costructures on the
generators as
\begin{align}
\Delta(\xi_i)&=\xi_i \otimes \one + \one \otimes \xi_i,\\
\epsilon(\xi_i)&=0,\\
S(\xi_i)&=-\xi_i,
\end{align}
and demanding that $\Delta,\epsilon$ are mutiplicative, i.e. $\Delta(\xi \xi^{\prime})=\Delta(\xi)\Delta(\xi^{\prime})$ and
$\epsilon(\xi \xi^{\prime})=\epsilon(\xi)\epsilon(\xi^{\prime})$, wherease $S$ is antimultiplicative. For example, to check that coproduct $\Delta$
makes sense, one must verify consistency of the following two expressions,
\begin{equation}
\Delta([\xi,\xi^{\prime}])=[\xi,\xi^{\prime}]\otimes \one + \one \otimes [\xi,\xi^{\prime}],\qquad
\Delta[\xi,\xi^{\prime}]=\Delta(\xi)\Delta(\xi^{\prime}) - \Delta(\xi^{\prime})\Delta(\xi).
\label{eqn:consistency}
\end{equation}

Apparently, despite a Hopf algebra $\cal{U}(\frak{g})$ is noncommutative, it is cocommutative. Namely, for two elements $\xi\in \cal{U}(\frak{g})$
(writing $\Delta(\xi)=\xi_{1}\otimes \xi_{2}$)
\begin{equation}
\xi_{1}\otimes \xi_{2}=\xi_{2}\otimes \xi_{1},
\label{eqn:Ug_cocommutativity}
\end{equation}
or equivalently, using the definition of opposite coproduct $\Delta^{\rm{op}}:=\Pi\circ \Delta$, $\Delta^{\rm{op}}(\xi)=\Delta(\xi)$.
Hopf algebras with such property are \textit{cocommutative triangular} ones. They are associated with Lie symmetries.

The idea of quantum algebras is so appropriately generalize trivial Hopf algebras $\cal{H}\cong \cal{U}(\frak{g})$.
Drinfel'd introduced a notion of \textit{almost cocommutative} Hopf algebra by proposing an invertible element $\cal{R}\in \cal{H}\otimes \cal{H}$,
expressing similarity of a coproduct and its opposite counterpart,
\begin{equation}
\Delta^{\rm{op}} = \cal{R}\Delta \cal{R}^{-1}.
\label{eqn:quasitriangularity}
\end{equation}
Then, Hopf algebra $\cal{H}$ is called \textit{quasi-triangular} if in addition the following two relations
\begin{align}
(\Delta \otimes \id)\cal{R}&=\cal{R}_{13}\cal{R}_{23},\\
(\id \otimes \Delta)\cal{R}&=\cal{R}_{13}\cal{R}_{12},
\end{align}
hold, using covariant expansions $\cal{R}_{12}=\cal{R}^{i}\otimes \cal{R}_{i}\otimes \one$,
$\cal{R}_{23}=\one \otimes \cal{R}^{i}\otimes \cal{R}_{i}$ and $\cal{R}_{13}=\cal{R}^{i}\otimes \one \otimes \cal{R}_{i}$ for
embeddings of a map $\cal{R}$ into $\cal{H}\otimes \cal{H}\otimes \cal{H}$.
As a consequence of \eqref{eqn:quasitriangularity}, $\cal{R}$ obeys a \textit{universal Yang-Baxter equation},
\begin{equation}
\boxed{\cal{R}_{12}\cal{R}_{13}\cal{R}_{23}=\cal{R}_{23}\cal{R}_{13}\cal{R}_{12},}
\end{equation}
which establishes main connection to the theory of quantum integrability. The element $\cal{R}$ is called the universal $R$-matrix.

Non-trivial quantum group can be understood as a deformation of $\cal{U}(\frak{g})$ achieved after appropriate twisting procedure.
Introducing an invertible twist element $\cal{F}$ from $\cal{U}(\frak{g})\otimes \cal{U}(\frak{g})$, which fulfills a cocycle condition
\begin{align}
(\cal{F}\otimes \one)(\Delta \otimes \id)\cal{F}&=(\one \otimes \cal{F})(\id \otimes \Delta),\\
(\epsilon \otimes \id)\cal{F}&=(\id \otimes \epsilon)\cal{F}=\one.
\end{align}
Its purpose is to define a new coproduct, $\Delta^{\cal{F}}:\cal{U}(\frak{g})\rightarrow \cal{U}(\frak{g})\otimes \cal{U}(\frak{g})$,
which is no longer cocommutative. In fact, $\Delta^{\cal{F}}$ is defined via similarity transformation on original coproduct $\Delta$,
\begin{equation}
\Delta^{\cal{F}}=\cal{F}\Delta \cal{F}^{-1}.
\end{equation}
Universal $\cal{R}$-matrix in the twisted Hopf algebra (quantum group) $\cal{U}_{\cal{F}}(\frak{g})$ is then expressed as
$\cal{R}=\cal{F}_{21}\cal{F}^{-1}$.

\paragraph{Example: deformation of $\frak{sl}_{2}(\CC)$.}
Consider an enveloping algebra $\cal{U}(\frak{sl}_{2})$, with Lie algebra generators $\{X^{+},X^{-},H\}$ subjected to commutation relations
\begin{equation}
[X^{+},X^{-}]=H,\quad [H,X^{\pm}]=\pm2X^{\pm}.
\label{eqn:sl2_commutation}
\end{equation}
The $q$-deformed Hopf algebra $\cal{U}_{q}(\frak{sl}_{2})$ is generated by elements $\{K_{+},K_{-},X_{+},X_{-}\}$ and unit element $1$,
satisfying deformed commutation relations
\begin{align}
[X_{+},X_{-}]&=\frac{K^{2}_{+}-K^{2}_{-}}{q-q^{-1}},\\
K_{+}X_{\pm}K_{-}&=q^{\pm 1}X_{\pm},\\
K_{+}K_{-}&=K_{-}K_{+}=1.
\label{eqn:Uqsl2_commutation}
\end{align}
Deformation parameter $q$, which can be arbitrary complex number $q\in \CC$, is defined such that in the $q\to 1$ limit \eqref{eqn:Uqsl2_commutation}
recovers undeformed $\frak{sl_2}$ commutation relation. This can be seen by formally taking $q=e^{\ii \hbar}$ and considering expansion of the
generators $K_{\pm}=e^{\pm \ii H/2}$ at $\cal{O}(\hbar)$. Algebra $\cal{U}_{q}(\frak{sl}_{2})$ becomes a Hopf algebra with the following costructures,
\begin{align}
\Delta(X_{\pm})&=X_{\pm}\otimes K_{+} + K_{-}\otimes X_{\pm},\quad \Delta(K_{\pm})=K_{\pm}\otimes K_{\pm},\\
\epsilon(X_{\pm})&=0,\quad \epsilon(K_{\pm})=1,\\
S(X_{\pm})&=-q^{\pm 1}X_{\pm},\quad S(K_{\pm})=K_{\mp}.
\end{align}
The amount of noncocommutativity is controlled by universal $\cal{R}$-matrix
$\cal{R}\in \cal{U}_{q}(\frak{sl}_{2})\otimes \cal{U}_{q}(\frak{sl}_{2})$,
\begin{equation}
\Delta^{\rm{op}}(a)=\cal{R}\Delta(a)\cal{R}^{-1},\qquad \forall a\in \cal{U}(\frak{sl}_{2}),
\end{equation}
reading explicitly
\begin{equation}
\cal{R}=q^{\frac{H\otimes H}{2}}\sum_{n=0}^{\infty}q^{n(n-1)/2}\frac{(1-q^{-2})^{n}}{[n]_{q}!}\left(q^{H/2}X_{+}\otimes q^{-H/2}X_{-}\right)^{n},\quad
[n]_q:=\frac{q^{n}-q^{-n}}{q-q^{-1}}.
\label{eqn:universal_R_matrix}
\end{equation}

\paragraph{Duality.}
The definition of Hopf algebra reflects its \textit{self-duality}.
In general, to a finite-dimensional Hopf algebra $\cal{H}$, one defines a dual Hopf algebra $\cal{H}^{*}$ via \textit{duality conditions},
\begin{align}
\expect{\alpha \beta,a}=\expect{\alpha \otimes \beta,\Delta(a)},\quad \expect{\one,a}=\epsilon(a),\\
\expect{\Delta(\alpha),a\otimes b}=\expect{\alpha,ab},\quad \epsilon(\alpha)=\expect{\alpha,\one},\\
\expect{S(\alpha),a}=\expect{\alpha,S(a)},
\label{eqn:duality_relations}
\end{align}
$\forall a,b\in \cal{H}$ and $\forall \alpha,\beta \in \cal{H}^{*}$, using notation $\alpha(a)\equiv \expect{\alpha,a}$ such that
$\expect{\alpha\otimes \beta,a\otimes b}=\expect{\alpha,a}\expect{\beta,b}$.
Relations \eqref{eqn:duality_relations} connect structures of $\cal{H}$ with costructures of $\cal{H}^{*}$, and vice-versa.
What is of special importance is that this duality persists even in the deformed case, when algebra $\frak{g}$ and corresponding group $G$ do
no longer exist.
For instance, the dual of $\cal{U}_{q}(\frak{sl}_{2}(\CC))$ is $\rm{Fun}_{q}(SL(2,\CC))$, namely a deformed Hopf algebra of functions over group
$SL(2,\CC)$ (which now, to some extent, justifies the name quantum group). This duality is directly manifest in the Faddeev-Reshetikhin-Takhtajan construction of quantum groups, elucidating formal
meaning of central algebraic relations in QISM, namely the RTT equation and the RLL equation [see appendix].

% references to add: textbook of Aschieri

\paragraph{Twists.}
Describe how new quantum groups are obtained via universal twists.
